Verify Before You Distill: Prompt-Level Teacher Gating for On-Policy Distillation

On-policy distillation (OPD) accelerates post-training by providing dense token-level supervision from a frozen teacher on the student's own rollouts. Vanilla OPD applies this supervision uniformly across prompts, without checking whether the teacher is reliable for each prompt. Because reverse KL is mode-seeking, a confidently wrong teacher can induce a strong yet misleading update. Distributional proxies, such as entropy or teacher-student likelihood agreement, measure uncertainty or agreement but do not directly verify outcome correctness. We introduce Teacher-Gated On-Policy Distillation (TGOPD), built on the principle that teacher reliability should be verified at the prompt level before dense supervision is admitted. TGOPD estimates reliability from a small set of verifier-scored teacher probes and routes each prompt exclusively to dense OPD when the reliability check passes or to verifier-grounded GRPO otherwise. Across 4B and 35B students in mathematics, code, and instruction following, TGOPD outperforms Vanilla OPD in all six single-domain settings and achieves higher seven-benchmark averages at both scales under multi-domain training. By using otherwise-idle teacher capacity for reliability estimation, TGOPD also reduces teacher-side compute waste in asynchronous OPD, increasing teacher-node GPU utilization from 9.8% to 78.9% in the measured 4B single-domain run.

==> sections/report-body.tex <==
\section{Why We Study Intelligence in the Wild}

In recent years, the progress of foundation models has often been observed through standard benchmarks, leaderboards, and controlled tasks. But real-world problems rarely arrive in benchmark form. A user may not know how to ask the perfect question; the meaning of a piece of content may be distributed across image, text, tone, and context; a safety decision may require evidence, rule hierarchy, and boundary judgment. These are not edge cases. They are the everyday conditions under which useful intelligence must operate, and they reveal a simple fact: many capabilities that are tested separately in benchmarks become \emph{entangled} in real systems. Agent systems make this entanglement especially visible by interleaving reasoning, environment actions, and external tools \citep{schick2023toolformerlanguagemodelsteach,yao2023reactsynergizingreasoningacting}.

To study Intelligence in the Wild is to study how these capabilities interact inside real systems. We treat real industrial scenarios as research fields: they expose failure modes that static evaluations often miss, and they provide new training signals, evaluation methods, and system boundaries for model evolution.

\section{The AllSpark Evaluation Loop}

Our central methodology is a closed loop that turns production experience into model improvement: a failure becomes a case; a case becomes a rubric; a rubric becomes an executable evaluator; an evaluator enters a benchmark, a reward signal, or a regression gate. Agent trajectories become training data, and production problems become new research questions.

\subsection{From Cases to Executable Rubrics}

Each rubric encodes what a good response must satisfy in a given scenario, expressed as checks that a judge model can execute against grounded evidence. Rubrics are versioned, reviewed, and promoted into regression suites once they discriminate reliably between strong and weak behavior.

\subsection{Pevek-1: A Foundation Model in the Wild}

We instantiate the loop with \textbf{Pevek-1}, a foundation model trained with a mixture of curated corpora, rubric-guided preference data, and agent-trajectory distillation. Below we report \emph{illustrative} results; all numbers are fake and included only to demonstrate the template.

\section{Experiments}

\subsection{Benchmarks}

We evaluate across a broad set of agentic-coding, search, reasoning, and tool-use suites, including software-engineering tasks inspired by SWE-bench \citep{jimenez2024swebenchlanguagemodelsresolve}. Figure~\ref{fig:benchmark-comparison} (page~1) summarizes the head-to-head comparison against leading models, and Table~\ref{tab:main-results} breaks the scores down by task group.

\subsection{Main Results}

Table~\ref{tab:main-results} reports the main comparison. Pevek-1 leads on every axis, with the largest margins on safety and agentic tool use, where rubric-guided feedback is most valuable.

\begin{table}[H]
\centering\small\color{abyss}
\setlength{\tabcolsep}{5.5pt}
\renewcommand{\arraystretch}{1.15}
\caption{Illustrative results by task (fake data).}
\label{tab:main-results}
\vspace{8pt}
\setlength{\aboverulesep}{0pt}\setlength{\belowrulesep}{0pt}
\begin{tabular}{l c c c c c}
\toprule
\textbf{Benchmark} & \textbf{Pevek-1} & \textbf{Kimi} & \textbf{GLM} & \textbf{GPT-5} & \textbf{Claude} \\
\midrule
\textit{Agentic Coding} & & & & & \\
SWE-Bench      & 57.9 & 63.5 & 62.1 & 58.6 & 69.2 \\
Terminal-Bench & 71.7 & 63.5 & 81.0 & 84.0 & 74.0 \\
NL2Repo        & 45.6 & 42.7 & 48.9 & 50.7 & 33.4 \\
\midrule
\textit{Agentic Search} & & & & & \\
BrowseComp     & 84.2 & 76.1 & 79.3 & 84.4 & 84.3 \\
WideSearch     & 76.4 & 74.3 & 72.3 & 80.0 & 72.9 \\
DeepSearchQA   & 91.0 & 87.7 & 89.1 & 95.5 & 93.1 \\
\midrule
\textit{Reasoning} & & & & & \\
GPQA-Diamond   & 90.4 & 88.1 & 86.2 & 93.6 & 93.6 \\
HLE            & 53.2 & 48.2 & 52.3 & 52.2 & 57.9 \\
MathArena      & 72.0 & 59.2 & 57.9 & 85.4 & 92.9 \\
\midrule
\textit{Tool Use} & & & & & \\
Tool-Decathlon & 48.5 & 47.8 & 40.7 & 55.6 & 59.9 \\
MCP-Atlas      & 79.1 & 73.6 & 71.8 & 81.6 & 82.2 \\
WebArena       & 53.6 & 43.5 & 48.7 & 63.2 & 58.4 \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Training Dynamics}

Figure~\ref{fig:training-dynamics} summarizes training dynamics and cost.
The left panel shows how the average evaluation score evolves, while the right panel reports the illustrative token cost required to reach three target scores.
Lower values are better in the right panel.

Both runs improve most rapidly during the first 30k training steps, but the rubric-guided run makes more progress in this early phase. At 20k steps, its average score reaches 60, compared with 55 for the baseline. The difference continues to grow as training proceeds, increasing from one point at initialization to eight points at 100k steps. This pattern indicates that the rubric-guided signal affects both learning speed and the final level reached by the model.

The shape of the curve is also informative. The rubric-guided run continues to improve through the middle of training and begins to flatten after roughly 70k steps. The baseline follows a similar schedule but enters a lower plateau. The smooth trajectories in this illustrative example make it possible to distinguish a persistent improvement from a temporary fluctuation at a single checkpoint.

Aggregate training curves should be interpreted together with task-level results. An average score can conceal regressions on individual capabilities even when the overall trend is positive. We therefore use the curve to identify when performance changes and the benchmark breakdown in Table~\ref{tab:main-results} to determine where those changes occur. In a complete model report, the same analysis would also include repeated runs and uncertainty estimates before selecting the final checkpoint.

Checkpoint selection should also account for stability near the plateau. Neighboring checkpoints can have similar aggregate scores while differing on individual tasks, inference cost, or robustness across repeated evaluations. We would therefore compare several checkpoints from the final phase of training on a held-out evaluation set rather than select the checkpoint with the highest single measurement. This procedure reduces sensitivity to evaluation noise and makes the reported endpoint easier to reproduce.

The evaluation protocol must remain fixed for the curve to support a training comparison. Each checkpoint should be evaluated with the same task set, prompts, tool configuration, scoring rules, and aggregation procedure. Failed or missing evaluations should also be handled consistently across checkpoints. Otherwise, a change in benchmark coverage or judge behavior can appear as model improvement. A complete report should therefore associate every point with a versioned evaluation configuration and retain the underlying task-level records for audit.

The right panel adds token cost to the stopping decision.
In this illustrative comparison, the rubric-guided run reaches the same target scores with fewer tokens than the baseline.

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{figures/training-dynamics}
\caption{Illustrative training dynamics and cost (fake data): average evaluation score across training steps (left) and tokens required to reach target scores (right).}
\label{fig:training-dynamics}
\end{figure}

\section{From Here}

The next stage of this work is to make the evaluation loop dependable across the full life cycle of a foundation model.
Intelligence in the Wild requires more than a strong aggregate score.
A useful model must remain reliable when prompts are incomplete, evidence is distributed across modalities, tools fail, and policies impose constraints.
We will therefore evaluate capability, robustness, efficiency, and safety together rather than treat them as independent endpoints.

Better coverage begins with real cases.
Production failures, difficult user interactions, and expert reviews can reveal combinations of capabilities that a static benchmark does not capture.
We plan to turn these cases into versioned rubrics and executable evaluations, while preserving the evidence needed to understand each judgment.
New cases will be separated from the data used for training so that the evaluation remains informative as the model improves.
This process should make benchmark growth traceable instead of allowing the test set to change without a record of why it changed.

Evaluation should then feed directly into training decisions.
For each intervention, we will compare the targeted improvement with changes on held-out task groups, repeated runs, and cost measures.
This comparison is necessary because a method can raise an average score while introducing a regression on a smaller but important capability.
Training curves, task-level breakdowns, and qualitative error analysis will therefore be reviewed together.
The resulting evidence can guide data selection, rubric revision, checkpoint selection, and decisions about when additional training no longer provides a useful return.

Deployment also needs an auditable feedback path.
Model outputs, tool interactions, evaluator decisions, and human corrections should be connected without removing the context required for interpretation.
At the same time, this record must respect privacy, access controls, and retention limits.
We will use the feedback path to distinguish model errors from tool failures, ambiguous instructions, and evaluation defects.
That distinction matters because these failure sources require different responses, and mixing them produces training signals that are difficult to trust.

Open collaboration can strengthen this process.
We intend to publish clear evaluation protocols, representative examples, and the assumptions behind reported results whenever the underlying data permits.
External challenge sets and independent reproductions can test whether an improvement transfers beyond the environment in which it was first observed.
They can also expose blind spots in our rubrics and help establish shared standards for evaluating models that act through tools and interact with people.

Our objective is a repeatable research process in which real-world evidence improves evaluation, evaluation improves training, and each reported gain can be inspected.
This is how AllSpark Research will continue to study intelligence in the wild.

